Software Architecture for Quantum Computing Systems -- A Systematic Review

Quantum computing systems rely on the principles of quantum mechanics to perform a multitude of computationally challenging tasks more efficiently than their classical counterparts. The architecture of software-intensive systems can empower architects who can leverage architecture-centric processes, practices, description languages, etc., to model, develop, and evolve quantum computing software (quantum software for short) at higher abstraction levels. We conducted a systematic literature review (SLR) to investigate (i) architectural process, (ii) modeling notations, (iii) architecture design patterns, (iv) tool support, and (iv) challenging factors for quantum software architecture. Results of the SLR indicate that quantum software represents a new genre of software-intensive systems; however, existing processes and notations can be tailored to derive the architecting activities and develop modeling languages for quantum software. Quantum bits (Qubits) mapped to Quantum gates (Qugates) can be represented as architectural components and connectors that implement quantum software. Tool-chains can incorporate reusable knowledge and human roles (e.g., quantum domain engineers, quantum code developers) to automate and customize the architectural process. Results of this SLR can facilitate researchers and practitioners to develop new hypotheses to be tested, derive reference architectures, and leverage architecture-centric principles and practices to engineer emerging and next generations of quantum software.

==> Context1.tex <==
\section{Background}
    This section contextualize some basic concepts including quantum computing, quantum software engineering and quantum software architecture \textcolor{red}{(see Figure \ref{QC}}). 

\subsection{Quantum Computing}
The field of Quantum computing (QC) has received rapidly growing industrial and policy interest to an even greater extent. It is evidenced by the fact that technology giants such as IBM, Google, and Microsoft have heavily invested in and committed to QC. However, cost-effectively, intuitively, and efficiently developing highly dependable QC applications is exceptionally challenging and remains an unsolved problem. However, solving this problem is critical to enable QC to live up to its promising potential.

QC is a fast growing research field and is expected to bring revolution in various industrial areas \cite{zhao2020quantum}. QC uses the concepts of quantum mechanics to process the information and complete specific tasks much faster than the classical computers. The quantum physics characteristics such as superposition, entanglement, and quantum interference are used and apply for computing purposes.Quantum computers outperform in two different ways as compared to the classical computers: 1) when the problem needs large amounts of parallel computing, e.g. big data analysis \cite{rebentrost2014quantum}\cite{zhao2020quantum}, data security \cite{zhao2020quantum}, encryption \cite{mosca2018cybersecurity}  and machine learning \cite{biamonte2017quantum}. 2) when the problem requires precise and effective computation in natural science e.g. physics \cite{childs2018toward} , material science \cite{grimsley2019adaptive} and chemistry \cite{mcardle2020quantum}.


From system’s engineering perspective, fundamental to quantum computing hardware is the concept of Qubit (quantum bit) that represent the most fundamental unit of quantum information processing [-]. Contrary to the classical bit (binary digit) that is expressed as (1, 0) in digital computing systems, Qubit as the quantum counterpart of bit is expressed as |0⟩ and |1⟩as shown in Figure \ref{QC}. The combinations of bits represent flow of digital information that alters the state of binary logic gates (on: 1 off: 0) to make digital systems work. Analogous to binary gates, quantum gate (a.k.a. quantum logic), as the building blocks of a quantum circuit transition its state via Qubit [-]. \textcolor{red}{The value zero is represented as} |0⟩ = [■(1@0)] and the value one is represented as |1⟩ = [■(0@1)]. \textcolor{red}{A quantum gate can have only one input and one output (transition of a single quantum state), or it can have multiple inputs and multiple outputs (transition of multiple quantum states).} The vector representation of a single qubit is:

 \begin{equation}
\big |a\rangle  =v01 \begin{bmatrix}
1 \\
0 
\end{bmatrix}   \big |1\rangle  = \begin{bmatrix}
0 \\
1 
\end{bmatrix}
\end{equation}


\begin{figure}[h!]
 \centering
%\setlength{\fboxrule}{1pt}
 \fbox{\includegraphics[scale=0.65]{Images/Context-Update.pdf}} 
 	\caption{A Simplified View of Quantum Computing Systems
([a] Quantum Hardware, [b] Quantum Software, [c] Quantum Software Architecture)
}
	\label{QC}
\end{figure}


Further details about Qubit and Qgate can be found in []. Like the classical computing systems, controlling the Qubits (to manipulating Qgate), there is a need for quantum software systems and applications that can exploit benefits of quantum information processing by operationalising quantum computers. For example, QuNetSim [] as a Python software framework manages quantum circuits to simulate processing and transmission of quantum information via quantum networks. However, in order to enable quantum software applications to utilise quantum hardware, there is a need for quantum code compilers that can translate high-level computational instructions into machine translated code to control quantum hardware []. As a typical example of such compilation, the solution in [] proposes a 2-layered architecture that receives the high-level source code (from programmer layer) and, automatically transforms it into the equivalent quantum representative source code (compilation layer). The compiled code can be executed or their underlying quantum algorithms can be simulated on quantum platforms to enable quantum processing to optimise solutions for unstructured data searching, parallel processing, and nature inspired computing. In recent years, a plethora of research and development has emerged that have focused on quantum algorithms [] and programming languages to address the above-mentioned computational challenges effectively and efficiently []. Despite the significance of quantum programming languages to produce executable specifications for quantum hardware; there is a need for overall engineering lifecycle(s) that goes beyond level of source code to specify, execute, validate and evolve software-intensive system based on required functionality and desired quality. 


\begin{comment}
\subsection{Quantum Software Engineering (QSE)}
Quantum computing is a technological revolution that demands a new software engineering paradigm to develop and conceive quantum software systems. Quantum software engineering calls for novel techniques, tools, processes and methods that explicitly focus on developing software systems based on quantum mechanics. SE activities, as presented in \textcolor{red}{Figure \ref{QC}} represent a simplified view of SE process adopted from \cite{zhao2020quantum} and such generalised process can be tailored (adding, removing, and/or customising any activities) as per the context of system development. In the following sections, we briefly discuss the quantum software development life-cycle phases \textit{(i.e. quantum software requirements engineering, quantum software design, quantum software implementation, quantum software testing, and quantum software maintenance)}  based on discussions available in existing studies.
\subsubsection{Quantum Software Requirements Engineering} \label{QSRE}
It is preliminary based on the concepts of classical software requirements engineering process, where functional, non-functional and system requirements are discussed. The quantum requirements analysis will continue through later phases of the development life cycle i.e. design, implementation, testing and maintenance. However, still no research work has been done that particularly focused on developing quantum requirements analysis techniques, tools and methodologies \cite{zhao2020quantum}. 

\subsubsection{Quantum Software Design} \label{Quantum Design}
 Similar to classical \cite{merlin1997SE}, the quantum software design involved two major phases i.e. architectural design and detail design. Architectural design is the abstract level design of quantum software, where the interactions of the main components are described \cite{zhao2020quantum}. The detailed design explicitly describes the data structure, algorithms, and the interfaces for module interactions. 
Developing algorithms for quantum software design is challenging as compared to the classical software systems because of some fundamental quantum computing features including superposition and entanglement. 

\subsubsection{Quantum Software Implementation} \label{Implementation}
Implementation -- or quantum programming -- is comparatively mature phase and considerable work is done on quantum programming languages \cite{chong2017programming}\cite{garhwal2021quantum}\cite{gay2006quantum}\cite{sofge2008survey}. It is important to select the most appropriate  programming technique based on the quantum application. There are number of quantum programming languages i.e. C (QCL), C++ (Scafflod), C\# (Q\#), Python (ProjectQ, Qiskit, Forest), F\# (LIQUi|⟩), Scala (Chisel-Q), and Haskell (Quiper). Therefore, the first critical step is to select the suitable programming technique that supports the given programming languages.

\subsubsection{Quantum Software Testing}\label{testing}
The testing phase begins to find defects and verify the system behavior. It might be possible that the programmers make various mistakes when they perform the quantum software testing because quantum computers have different properties such as superposition, entanglement and no cloning \cite{national2019quantum}\cite{zhao2020quantum}, which make challenging to predict the behavior of the quantum software \cite{chong2017programming}\cite{ying2016foundations}. There is a strong need for different testing tools and techniques that consider the mentioned quantum computing characteristics \cite{stepney2005journeys}.

\subsubsection{Quantum Software Maintenance} \label{maintenance}
The maintenance phase includes updating, changing and modifying the quantum software to keep up with the customer needs. This is an emerging research area in quantum software engineering \cite{kruger2020quantum}\cite{perez2020reengineering}, which specifically focuses on re-engineering the available classical information systems and their integration with the quantum algorithms. In the short term, quantum computers might not be able to give full-fledged features because of high cost, lack of processes, tools and techniques. However, the concept of migrating the quantum algorithms to the existing classical information systems is the best option.  Therefore, it is important to revisit the reengineering (maintenance) concepts to deal with the migration process.
\end{comment}

\subsection{Quantum Software Engineering (SE)}
Software engineering as an ISO/IEC/IEEE 90003:2018 standard aims to apply engineering principle and practices to design, develop, validate, deploy and evolve software-intensive systems effectively []. In recent years, SE focused research and development started to tackle software related challenges, i.e., quantum software models [], their algorithmic specifications [], and simulated evaluations [] to leverage benefits of quantum hardware for quantum information processing. More specifically, software engineers can leverage SE practices and patterns by following software process(es) that comprises of a multitude of engineering activities including but not limited to requirements engineering, design, implementation, evaluation, and deployment, as in Figure \ref{QC}. SE activities, as presented in Figure \ref{QC} represent a simplified view of SE process adopted from [] and such generalised process can be tailored (adding, removing, and/or customising any activities) as per the context of system development. Quantum computing systems are in a phase of continuous evolution and consequently quantum SE represents a new genre of software-intensive engineering activities to develop applications that can control the underlying hardware. In addition to the needs for innovative SE processes, principle, and practices that specifically tackle challenges for quantum modeling and architecting [], coding, and simulation [], existing classical SE processes can be customized to engineer and develop quantum software. For example, the concept of architectural modeling as generic SE activity, can be customised with initiatives like QML that models parallel computing for quantum search algorithms []. Similarly, existing requirements engineering process can be tailored to accommodate quantum requirements (i.e., entanglement) that is missing in existing models. In SE process(es), architecting represents a pivotal activity that accumulates system requirements as a model that leads to software implementation, validation, and evolution while maintaining a global view of the system and managing architectural trade-offs [].  




\subsection{Architecture for Quantum Software}
ISO/IEC/IEEE 42010:2011 \cite{ISO/IEC} aims to abstract complex and implementation specific details of system in terms of architectural components and connectors to represent system in implementation and technology neutral way. Specifically, source code modules of a software can be represented as architectural components (units of computation and storage), while module interconnections can be represented as architectural connectors (coordinating components) to model a system while abstracting complex details of implementations. Once expressed, architectural models, i.e., model driven architecture [] can helps to generate the necessary skeleton or libraries of source code in a (semi-) automated way using model-driven engineering []. \\   
In recent years, architectural models and notations have proven to be successful to design and develop software-intensive systems by enabling reusability [] (patterns and styles), evolvability [] (architectural reconfigurations), and elasticity [] (auto-scaling). In \textcolor{red}{Figure \ref{QC}}, for illustrative purposes, a partial architectural view of a quantum algorithm to search unstructured data is presented using UML component diagram []. The architectural view abstracts the source coding level details to present design decision in terms of components () that coordinate to find a number […]. Architecture in itself represent non-executable specifications of the quantum search system, however; the application of model-driven engineering can help architects and designers to derive source code directly from architecture models.

In the overall view of \textcolor{red}{Figure \ref{QC}}, we can conclude that in quantum computing systems, software architecture represents a blue-print to develop software systems and applications that manipulate quantum hardware. Specifically, the role of software architecture in quantum SE is pivotal to model requirements leading to software modeling, coding, validation and deployment all facilitated using architectural notations.  Software architecture for quantum computing systems (Quantum software architecture) can empower the role of software engineers and developers to create models that acts as basis for system implementation. Based on the architectural model, model driven engineering and development can be exploited for the automated generation of the source code (code modules and their interactions) from the corresponding architecture (based on architectural component and their connectors).




==> Discussions.tex <==
\section{Discussions} \label{discussions}
We now summarise the core findings and key results of the SLR - consisting answers to all RQs -  to reiterate state-of-research on architecting quantum software. Conclusive summary of each RQ is presented in dedicated subsections below. 

\subsection{Research status (RQ1.1)}
Year based publication results of the selected studies are discussed in Section \ref{RQ1.1}. We see an upward trend in the number of publications on quantum software architecture (see Figure \ref{Fig:Frequencyandpublicationtype}). The bar graph reveals that since 2018 there has been a significant increase in the number of published studies, and \textit{(n=21, 62\%)} primary studies are published in the last three years. These results highlight the great interest of researchers and practitioners in quantum software architecture. The fast-growing number of research publications depicts quantum software architecture as an emerging research area, which is approaching the commercialization phase to achieve industrial breakthroughs and enables new business models. We further noticed that journals  \textit{(n=16, 47\%)} are the most common venues to publish quantum software architecture studies. Journals are mostly more selective and publish high-quality studies with deep analysis. This finding predict that most of the selected primary studies are of high quality and provide concrete insights based on their results and analysis.  

\subsection{Research types and contribution (RQ1.2)}
Systematic thematic classification of research types and contributions is provided in Figure \ref{Fig:Researchfacetsandfocus} (a). The selected studies are categorized across five core research-type facets proposed by Wieringa et al. \cite{wieringa2006requirements}. The review results reported in Section \ref{RQ1.2} illustrate that most of the studies \textit{(n=20, 59\%)} cover both proposal of solution and validation research types, which are jointly considered in the heterogeneous \textit{proposal of solution and validation research} type category. For instance, various studies contributed by presenting architectural solutions and tools with validation discussion for co-design (quantum and classical) systems [S16, S17, S18, S23, S24, S28]. For example, Wille et al. [S16] introduced a set of tools for quantum-classical co-design, which mainly tackles various design problems including compilation, verification, and simulation. These tools are empirically validated and made available as open-source for researchers and practitioners. Similarly, Li et al. [S2] designed a secure quantum key distribution (QKD) software architecture for data encryption in quantum networks. The simulation-based experiment was performed on the Windows platform to validate the significance of the proposed architecture. The quantum computing field is continuously evolving and that might be the reason that simulation is considered the most common validation approach, in contrast to classical computing, where architectural solutions are validated using case studies or experimental settings \cite{kumar2016software}.

Regarding selected primary studies contribution, we identified that a total \textit{(n=9, 27\%)} studies focused on \textit{co-design of the quantum systems} (see Figure \ref{Fig:Researchfacetsandfocus} (a)), where both classical and quantum techniques  are simultaneously optimised to develop the architectural solutions \cite{van2018co}. 
Quantum computing systems are highly fragile to environmental interruption, and this interruption brings uncertainty (decoherence) in the quantum state (i.e. superposition), which is probably high as compared to classical computations \cite{jeff2021}. Practical quantum computers are expected to have, at least at the interface level interaction with the classical computers. It could be realised by following the co-design architectural concepts, where hybrid architectures are developed both at the software and hardware levels \cite{jeff2021}. Presently, it is not possible to entirely ignore the classical computing attributes because of various technological, managerial, and organizational challenges in quantum computing domain. \\ 

\subsection{Application domains (RQ1.3)}

We conducted thematic classification of the selected primary studies across application domains (see Figure \ref{Fig:Researchfacetsandfocus} (b)). We observed that \textit{ (n=20, 59\%)} studies are mapped into the \textit{systems and hardware engineering} theme, which is the most dominating application domain. It exhibits that most of the selected studies are conducted with the aim to propose architectural solutions for both quantum software and hardware systems. It means that researchers are greatly intended to offer real-world architectural solutions. Even though quantum software and systems research is still pretty nascent, however, the competition in the field is ramping up. The leading contenders (e.g., China and USA) are racing to dominate and become the first to conquer the market. 

The second most common theme for application domains is \textit{software engineering}. Software is as important as hardware and it plays a critical role in powering the quantum revolution \cite{WinNTYehuda}. The quantum computing field will be entirely stalled without concrete progress in quantum software engineering research \cite{WinNTYehuda}. Quantum software systems will make it possible to run more advanced algorithms on sophisticated quantum computing machines. The big quantum computing promise is only possible by integrating hardware and software systems along with skilled workforce.

The quantum software architectural solutions are proposed in different areas; however, we realized that many application domains are still missing, e.g.,
\textit{model-driven quantum software architecture (MDQSA), quantum AI software architecture}  and \textit{quantum software architecture applications for the industrial problems}.


\subsection{Architectural process (RQ2.1)}
Architectural process enables software designers and architects to follow a structured approach to analyse, synthesise, and evaluate architecture-centric solution to develop software-intensive systems \cite{RQ1-1}. The available evidence about process(es) for architecting quantum software (extracted from 14 studies) such as [S2, S5, S14, S19] indicates five distinct activities as illustrated in Figure \ref{QSA}. These activities namely \textit{architectural requirements}, \textit{architectural modeling}, \textit{architectural implementation}, \textit{architectural validation}, and \textit{architectural deployment} support an incremental architecting of the quantum software. Incremental architecting refers to accumulating architectural knowledge from previous activity (e.g., architectural design) to support next activity in the process (e.g., architectural implementation) \cite{ RQ1-5}. QSA represents an innovative genre of software architectures, however; from a theoretical perspective architecting activities and the process that encapsulate these activities for QSA are based on existing architectural process for classical software systems \cite{ RQ1-1}\cite{RQ1-5}. However, in practice quantum specific architectural requirements such as quantum system co-design requires mapping of the Qubits to Qugates - exploiting domain specific models - to architectural components and connectors [S5, S7]. Based on the published research on architectural process for QSAs, architectural validation and deployment activities are mostly overlooked. There is need for further research that goes beyond architectural design and implementation to develop methods and solutions for architecture-centric validation, deployment, and maintenance of QSAs. 

\subsection{Architectural modeling notation (RQ2.2)}
 Architectural modeling notations provide graphical and descriptive specifications to model the architectures and add visual representation of software under design, as highlighted in Table \ref{tab:ModelingNotation}. The SLR suggests that existing research (based on evidence from 18 studies) exploits three main types of modeling notations to model QSAs. These notations include \textit{UML profiles and extensions}, \textit{graph-based models}, along with \textit{box and arrow} representations [S4, S9, S32,S2, S5, S7, S1, S6, S14]. Unlike architectural modeling for classical software systems that primarily rely on UML or architectural description languages, it appears that graph-based models and informal box and arrow structures are being used more frequently to model QSAs \cite{perez2021modelling}\cite{RQ1-5}[S7][S14]. Graph-based models provides a formal approach (based on graph theoretical foundations) to represents the structure and behavior of QSAs. In comparison, the informal box and arrow structures provide an intuitive mechanism (supporting circuit diagram) to model Qubits and their mapping to Qugates [S6, S21]. There is a need to exploit well established principle and practices from existing architectural languages that can be tailored to describe architecture for quantum software \cite{TSEADL}.  

\subsection{Architecture design patterns (RQ2.3)}
We noticed that a total of 6 quantum software architectural patterns are discussed in 16 primary studies (47.05\%) (see Table \ref{tab:QSEpatterns}). We observed that \textit{Layered} and \textit{Pipe and filter} are the most common architecture patterns to design quantum software. We realized that most of the studies repeatedly mentioned or used these patterns (i.e., \textit{Layered} and \textit{Pipe and filter}) in the context of quantum software which indicates that most of the architectural components of quantum software are similar to architectural components of classical software systems. The significant difference is regarding the execution behavior of the quantum instructions between quantum and classical software. For example, in layered pattern for quantum software, instructions are passed through several stages before reaching to host quantum computing CPU [S3]. The arbiter component fetches the instructions from the main memory and passes them to the quantum control unit. Quantum control unit processes the instructions within several parts (e.g., quantum instruction cache, Q-address translator, and Q symbol table). After processing in quantum control unit, instructions are moved to the physical execution layer via the Pauli Arbiter QEC cycle generator component. The physical execution layer has several parts (e.g., routing logic, timestamp manager, operations combination, timing controller, and binary feedback control), and instructions are going through every component. After processing the physical execution layer unit, instructions are moved to the quantum-classical interface, which generates the Qubits. These Qubits are sent back to the quantum control unit via the physical layer, and the quantum control unit sends the Qubits to the host CPU for execution. 
However, it is worthwhile to mention that most of the identified patterns are mainly used to design and implement the architecture of the small-scale quantum software systems. We did not find any other pattern specifically used for medium or large-scale quantum software systems. On the other hand, we also not find any study that discusses architectural framework for quantum software systems. To this end, further research is required to i) investigate and propose the architectural patterns for medium or large-scale quantum software systems, and ii) investigate the architectural framework for describing the architecture of quantum software systems.

\subsection{Architecture tools and frameworks (RQ2.4)} \label{RQ2.4Discussion}
Tools and frameworks play a significant role in the customization and automation of the solutions to minimize human errors and efforts. We explicitly explored the selected primary studies and identified 11 tools and frameworks for quantum software architecture. The identified tools are discussed based on five quality attributes  and presented a toolchain for automating the architecting activities \cite{sajjad2018classification} (see Section \ref{RQ2.4}).

The review reveals that most of the tools and frameworks are open source. It means that a wide range of available quantum software architecture tools and frameworks are freely available to the community for use and making possible improvement contributions. We further noticed that majority of the tools are capable of simulating the input of the existing high-level programming languages and giving quantum output. It magnifies the concept of hybrid (quantum-classical) computation model, where the existing high-level programming languages (e.g., C\#, Java, Python, C, C++ ) are used to develop the input code for quantum computations. Our observation is aligned with the hybrid quantum programming concept discussed by Zhao \cite{zhao2020quantum}, which consists of both classical and quantum components. Similarly, we realised that simulation findings (SF) is the most common output type of identified tools and frameworks (see Table \ref{tab:Tools}). It acknowledges the fact that large-scale quantum software architecture implementation is still challenging and the simulation findings are mainly used to validate the design of the proposed architectures. Moreover, most of the tools are fully automated that execute the high-level or quantum instructions and produce the quantum outputs. For example, XACC (eXtreme-scale ACCelerator) is a fully automated framework and it provide automation interface for integration and interoperability across the quantum programming landscapes [S4]. Additionally, we noticed that eight studies explicitly evaluated the significance of the proposed tools and frameworks (see Table \ref{tab:Tools}). For instance, the performance of QuNetSim is evaluated by examples and the clear instructions to execute the tool (i.e., code snippets explaining how to use a library or list of commands that should be executed in command line with an explanation of the arguments) are provided [S25]. 

Finally, we provided a toolchain used to customise and automate various architecting activities (see Section \ref{RQ2.4}, Figure \ref{Fig:Toolsupport}). We noticed that most of the tools and frameworks are developed for \textit{architectural implementation} activity. Quantum computing is an emerging field with significant potential across different areas including cybersecurity in finance industry, defense, weather forecasting, and healthcare by improving diagnoses and personalising medicines. However, establishing quantum software development field will take decades and it might be the reason that technology giants and startups are competing to bring the early solutions. They more focus on the implementation phase to provide preliminary quantum software platforms to end-users. In conclusion, it is vital to highlight that very few software tools and frameworks are available \textit{(11/34 studies, 32\%)} for supporting architecting activities, more specifically \textit{architectural requirements} and \textit{architectural deployment} are less focused areas. There is a demanding need of more advanced tools and frameworks to improve the efficiency and precision of architecting activities and minimizing the cost and effort of manual solutions.

\subsection{Architectural challenges (RQ2.5)} 
The selected primary studies are reviewed and analysed to identify the architecture challenges in quantum software systems. The review findings uncover a total of 15 challenging factors, which are further mapped across four core themes. The thematic mapping and description of the challenging factors is reported in Section \ref{RQ2.5}. Figure \ref{Fig:Challengesthemes} encapsulates the mapping results, which exhibit that most of the challenges are related to the \textit{(architectural tools and technologies; (n=6, 18\%)} theme. Compared to quantum hardware development, the quantum software architecture is a relatively new and less established field. Different tools and technologies are developed; however, these tools and technologies are adopted at a low level and still not strong enough to tackle the architectural issues \cite{gill2020quantum}. For instance, Noisy Intermediate-Scale Quantum (NISQ) computers is identified as the most common architectural challenge of \textit{architectural tools and technologies} theme [S21, S15]. The NISQ computers are not error-free, and their operations are imperfect and limited to a small number of qubits. It is hard to achieve the high number qubits computations using NISQ computers. Similarly, four challenging factors \textit{(n=4, 12\%)} are classified across the \textit{quantum data transmission and security} theme (see Section \ref{RQ2.5}). Quantum network security protects the network from security threats, data breaches, intrusions, and ensures secure data transfer and communication across interconnected entities. However, architecting and maintaining a secure quantum network is extremely challenging because of quantum cryptography, teleportation strategies, communication technologies, and quantum key distribution techniques. For instance, proposing an architectural solution for quantum cryptography is a significant quantum networks challenge because of transferring quantum states, secure encryption and decryption, public trust, cost, and sharing infrastructure. Presently, it is hard to address these challenges, and major technology giants across the world are trying their best to propose suitable quantum cryptography solutions. Moreover, three challenges are mapped into the \textit{process-centric architecting} theme. For example, architectural pattern selection is reported as an process-centric architecting challenging factor [S14, S33]. Selecting the most suitable pattern can entail various challenges. There is a demanding need for a decision-making model that could help to select appropriate architecture patterns. It will assist the practitioners in exploring a set of existing patterns and determine the most relevant pattern based on the architectural problem.

In summary, researchers and practitioners have demanding tasks ahead to prepare for the reported challenges, which can be potential barriers for quantum software architecture. To achieve the exciting benefits of quantum software systems, it is mandatory to mitigate the challenging factors. There is an open call for both researchers and practitioners to come forward and join this effort. 
